MatExPre: A matrix exponential preconditioner for the high-frequency Helmholtz equation

In this article, we present a new preconditioner, MatExPre, for the high-frequency Helmholtz equation by leveraging the properties of matrix exponentials. Our approach begins by reformulating the Helmholtz equation into a Schr\"{o}dinger-like equation and constructing a time-domain solver based on a fixed-point iteration. We then establish a rigorous connection between the time-domain solver and matrix exponential integrators, which enables us to derive algebraic preconditioners that rely solely on sparse matrix-vector products. Spectral analysis and a detailed numerical implementation strategy, including performance improvements achieved through complex shifting, are discussed. Finally, numerical experiments on 2D and large-scale 3D homogeneous and inhomogeneous models, including benchmark seismic examples, substantiate the effectiveness and scalability of the proposed methods.

==> siam_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
% \usepackage{lipsum}
% \usepackage{amsfonts}
% \usepackage{graphicx}
% \usepackage{epstopdf}
% \usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Personal latex commands should be portable for any template.
\input{latex-commands.tex}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}
\newsiamremark{fact}{Fact}
\crefname{fact}{Fact}{Facts}

% Sets running headers as well as PDF title and authors
\headers{MatExPre: A matrix exponential preconditioner}{S.\ Fu, Q.-H.\ Liu, Q.\ Zhan, E.\ T.\ Chung, and C.\ Ye}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{MatExPre: A matrix exponential preconditioner for the high-frequency Helmholtz equation\thanks{Submitted to the editors DATE.
    \funding{This work was funded by the Fog Research Institute under contract no.~FRI-454.}}}

% Authors: full names plus addresses.
\author{
  Shubin Fu\thanks{Eastern Institute of Technology, Ningbo, Zhejiang, 315200, China.
    \\(\email{sfu@eitech.edu.cn}, \email{qhliu@eitech.edu.cn})}
  \and Qing Huo Liu\footnotemark[2]
  \and Qiwei Zhan\thanks{College of Information Science and Electronic Engineering, Zhejiang University, Hangzhou, Zhejiang, China.
    (\email{qwzhan@zju.edu.cn})}
  \and Eric T.\ Chung\thanks{Department of Mathematics, The Chinese University of Hong Kong, Shatin, Hong Kong SAR, China.
    (\email{eric.t.chung@cuhk.edu.hk}, \email{changqingye@cuhk.edu.hk}).}
  \and Changqing~Ye\footnotemark[4]}

% \usepackage{amsopn}
% \DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

